Two-Leg Deep Space Relay Architectures: Performance, Challenges, and Perspectives

In this paper, architectures for interplanetary communications that feature the use of a data relay are investigated. In the considered "two-leg" architecture, a spacecraft orbiting the Earth, or in orbit at a Lagrange point, receives data from a deep space probe (leg-1) and relays them towards ground (leg-2). Different wireless technologies for the interplanetary link, namely, radio frequencies above the Ka band and optical frequencies, are considered. Moreover, the cases of transparent and regenerative relaying as well as different different orbital configurations are addressed, offering a thorough analysis of such systems from different viewpoints. Results show that, under certain constraints in terms of pointing accuracy and onboard antenna size, the adoption of a two-leg architecture can achieve the data rates supported by direct space-to-Earth link configurations with remarkably smaller ground station antennas.

==> Figures/Table_Summary_OLD.tex <==
\begin{table*}[!t]
\begin{center}
\caption{Analysis Outcomes and Architecture Recommendations.}\label{table:Outcomes}
\footnotesize{
\begin{tabular}{|p{5cm}|p{5cm}|p{5cm}|}
 \toprule
                  {\textbf{Direct Link}}  &     {\textbf{Optical Frequencies}}      &     {\textbf{EHF}}   \\  \toprule
                  
{\textbf{RF Power}: } & {\textbf{RF Power}: Pave = 5 W, Ppeak = 400 W} &  {\textbf{RF Power}: }  \\ & & \\ 

{\textbf{Deep Space Antenna}: } & {\textbf{Deep Space Antenna}: Optical antenna size of 1.39 m.} &  {\textbf{Deep Space Antenna}: on-board antenna diameter of approx. 5 m.}  \\ & & \\

 & {\textbf{Relay Satellite Antenna Leg1}: Optical antenna size of 1.39 m} &  {\textbf{Relay Satellite Antenna Leg1}:}  \\ & & \\

{\textbf{Frequencies}: } & {\textbf{Frequencies}: } &  {\textbf{Frequencies}: f1 = 43 GHz or more.}  \\ & & \\ 

{\textbf{Pointing requirements}: } & {\textbf{Pointing requirements}: 0.50 μrad (low noise) and 0.35 μrad (high noise) for Venus and Mars; 0.20 μrad (low noise) and 0.10 μrad (high noise) for Uranus and Neptune.} & {\textbf{Pointing requirements}: S/C pointing accuracy of 0.01°}\\ & & \\ 

{\textbf{Data rate}: } & {\textbf{Data rate Leg1}: } & {\textbf{Data rate Leg1}: } \\ & & \\ 

{\textbf{Ground Antenna}: the typical deep space antenna diameter has been considered = 35 m.} &  &  \\ 

\cmidrule[\heavyrulewidth]{2-3} 
                  & \multicolumn{2}{c|}{{\textbf{Leg2}}} \\ \cmidrule[\heavyrulewidth]{2-3} 
                  & \multicolumn{2}{p{11cm}|}{\textbf{Ground Antenna}: Small antennas can be employed on the ground segment side, 2.4 m for GEO or Lagrange L1 relay scenarios or approx. $10$ m for L$4$/L$5$ relay scenario} \\ 
                  & \multicolumn{2}{p{11cm}|}{}\\
                  & \multicolumn{2}{p{11cm}|}{\textbf{Relay Satellite Antenna Leg2}: } \\ 
                  & \multicolumn{2}{p{11cm}|}{}\\
                  & \multicolumn{2}{p{11cm}|}{\textbf{Data rate Leg2}: }  
                  \\ \bottomrule
\end{tabular}}
\end{center}
\end{table*}
